ConvoSense: Overcoming Monotonous Commonsense Inferences for Conversational AI

Mastering commonsense understanding and reasoning is a pivotal skill essential for conducting engaging conversations. While there have been several attempts to create datasets that facilitate commonsense inferences in dialogue contexts, existing datasets tend to lack in-depth details, restate information already present in the conversation, and often fail to capture the multifaceted nature of commonsense reasoning. In response to these limitations, we compile a new synthetic dataset for commonsense reasoning in dialogue contexts using GPT, ConvoSense, that boasts greater contextual novelty, offers a higher volume of inferences per example, and substantially enriches the detail conveyed by the inferences. Our dataset contains over 500,000 inferences across 12,000 dialogues with 10 popular inference types, which empowers the training of generative commonsense models for dialogue that are superior in producing plausible inferences with high novelty when compared to models trained on the previous datasets. To the best of our knowledge, ConvoSense is the first of its kind to provide such a multitude of novel inferences at such a large scale.

==> fig/eval-interface.tex <==

\begin{figure*}[ht]
\centering
\begin{subfigure}{\textwidth}
  \centering
  \includegraphics[width=\linewidth]{img/eval-instructions.png}
  \caption{Instructions}
  \label{fig:eval-instructions}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{img/eval-reasonable.png}
  \caption{Reasonability Q}
  \label{fig:eval-question-r}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{img/eval-novel.png}
  \caption{Novelty Q}
  \label{fig:eval-question-n}
\end{subfigure}
\caption{The instructions and questions shown to human evaluators for inference evaluation.}
\label{fig:eval-interface}
\end{figure*}

==> fig/results-by-type.tex <==

\begin{figure*}[t]
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{img/reasonability-comfact.pdf}
  \label{fig:reasonable-comfact}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=\linewidth]{img/reasonability-cicero.pdf}
  \label{fig:reasonable-cicero}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=\linewidth]{img/reasonability-reflect.pdf}
  \label{fig:reasonable-reflect}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{img/novelty-comfact.pdf}
  \label{fig:novel-comfact}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=\linewidth]{img/novelty-cicero.pdf}
  \label{fig:novel-cicero}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=\linewidth]{img/novelty-reflect.pdf}
  \label{fig:novel-reflect}
\end{subfigure}
\caption{\small Proportions of reasonable (top) and novel (bottom) inferences per inference type.}
\label{fig:results-by-type}
\end{figure*}

% -- the % symbol is affecting how the figures stay on a line together?!

==> sections/humangen.tex <==
\section{Existing Human-Generated Datasets}
\label{sec:existing_datasets}

In the rest of this work, we combine the existing human-generated commonsense datasets into a solitary dataset, denoted as \textbf{HumanGen}. HumanGen is constructed by concatenating the train/validation/test divisions of the datasets, using the provided splits for ComFact and Cicero and sampling Reflect in an 80/10/10 distribution. 

To standardize HumanGen into a cohesive format, we perform the following preprocessing steps. 
First, we leverage the mapping outlined in Table \ref{tab:human-gen-datasets-types} along with the specifications from Table \ref{tab:gpt-prompts} to identify relevant commonsense inference questions for each instance. Then, we combine consecutive dialogue utterances from the same speaker, thereby ensuring that each dialogue turn represents a distinct speaker.

Lastly, we apply the Speaker/Listener tags in a similar manner to ConvoSense (Sec. \ref{sec:convosense}). Given that human-generated inferences frequently contain nominal references to specific target entities, we additionally incorporate the names of conversational participants into the tags as exemplified by "Speaker (A)". However, the naming conventions vary across different human datasets. To maintain consistency, we adopt the naming conventions used in the Cicero dataset for both Reflect and Comfact datasets, as Cicero constitutes nearly 90\% of the human data. In Cicero, participants are denoted as A and B. For the Comfact dataset, which originally lacks speaker designations, we randomly assign A/B tags to each conversation. On the contrary, Reflect includes original speaker names (e.g., Jesse, Bailey, etc.), which we replace randomly with A/B tags. Moreover, considering that the speaker's name frequently appears in Reflect's inferences, we uniformly replace it with \texttt{"the speaker"}, aligning with the prevalent format in Cicero inferences.

% Almost 60\% of inferences in Cicero refer to the speaker as \texttt{"the speaker"}, whereas the remaining inferences tend to not specify the focal person.

==> sections/old/data-human-generated-old.tex <==
\section{Existing Datasets}
It has been a longstanding effort to produce commonsense inference datasets. Although the earliest works like the popular ConceptNet focused heavily on physical-entity-based commonsense, such as "tires are a part of a car", there has been more recent work on constructing datasets that address social- and event-based commonsense, rather than entity-based, such as ATOMIC. 

Since dialogue often focuses on social situations and life events, works like ATOMIC could contain information that is more directly relevant for dialogue applications. However, one major limitation of ATOMIC is that it has no contextual component, since it focuses on short, singular phrases as the premise for its commonsense inferences. This makes it difficult to utilize for dialogue tasks, such as producing commonsense inferences relevant to a specific utterance, since utterances cannot be treated as isolated and independent from one another. Rather, the long-form dialogue context is necessary to properly understand each singular utterance.

As a result, recent efforts have pushed to construct datasets that curate commonsense inferences applicable to dialogue contexts. These existing datasets are often restricted in scale for both their covered inference types and their diversity of dialogue contexts. Table \ref{tab:human-gen-datasets-scale} presents statistics on the scale of the datasets discussed in the rest of this section.

\input{tab/data-human-generated-scale}

% Sources:
% \textbf{Reflect} dialogues are taken from Commonsense-Dialogues, which are relatively short dialogues constructed around a specified social situation (e.g. "Tom overheard his friend Sydney's parents arguing about divorce").

\subsection{ATOMIC}

The ATOMIC datasets structure their commonsense as a premise (which is a short phrase describing some event), an inference type, and a reasonable inference that fits the definition of said type (which is also a short phrase like the premise). The highest quality ATOMIC dataset is the one called \textbf{ATOMIC10X$_{high}$} which was constructed from filtered results from GPT3 \cite{west:22}. First, human-generated examples of premises from the precursor dataset \textbf{ATOMIC2020} were used as in-context learning examples in the GPT3 prompt, and GPT3 was tasked with producing a large-scale set of additional premises. Then, similarly, each inference type from the precursor dataset \textbf{ATOMIC2020} were used as in-context learning examples in the GPT3 prompt, and GPT3 was tasked with producing more instances of each inference type for the previously generated premises. A classifier was developed to predict whether a commonsense inference was reasonable for its premise by training on 10,000 GPT3 generations annotated by humans for their reasonability. This classifier was then used to filter the large-scale GPT3 generations to produce the final \textbf{ATOMIC10X$_{high}$} dataset.


\subsection{ComFact}

The \textbf{ComFact} dataset \cite{gao:22} maps dialogue contexts to reasonable inferences from the existing \textbf{ATOMIC2020} dataset. For each utterance of every dialogue in the dataset, a list of candidate inferences is retrieved from \textbf{ATOMIC2020} using exact string matching and embedding similarity between the utterance and the premises of the commonsense inferences. Human annotators are then tasked with labelling the applicability of a commonsense inference to the utterance within its dialogue context, considering both historical dialogue context and future dialogue context. For the purposes of this work, only the human-annotated relevant inferences are considered.

% \subsection{Cider}

% Cider was the first work to produce a dataset that contains novel commonsense inferences for dialogue. Within Cider, pairs of utterances in a dialogue context were labelled by humans with derivable commonsense inferences. For example, in the pair of utterances ("SpeakerA: Why were you late for work?", "SpeakerB: I missed the bus"), the event "missed the bus" would be linked to the event "late for work" with a causal inference type. By design, Cider is restricted to contain only those inferences that are explicitly revealed in the dialogue and does not include any speculative commonsense inferences.

\subsection{Cicero}

Cicero was the first dataset to provide novel speculative commonsense inferences for dialogue contexts. Cicero tasked human participants with providing answers to 5 different commonsense questions (such as " What is an emotion or basic human drive that motivates or could motivate Target?") for various target utterances within specified dialogue contexts. The first version \textbf{Cicerov1} \cite{ghosal:22} produced a single positive inference for each inference type for each (target utterance, dialogue context) datapoint being annotated, whereas the later version \textbf{Cicerov2} \cite{shen:22} produced multiple positive and negative inferences for each to better model the polymorphism of speculative commonsense inferences. For the purposes of this work, only the positive inferences are considered.

\subsection{Reflect}

The \textbf{Reflect} dataset \cite{zhou:22} provides both human-generated commonsense inferences for a dialogue context as well as next-utterance responses that are derivable from a specified commonsense inference. Similarly to \textbf{Cicerov1/2}, human participants provide commonsense inferences for a dialogue context by answering a commonsense question. As a separate task, new human participants are then instructed to construct a reasonable next-utterance response to the given dialogue context that stems from a provided commonsense inference.

\section{Inference Types for Dialogue}
\label{sec:type_synthesis}

\input{tab/data-human-generated-types}

Table \ref{tab:human-gen-datasets-types} summarizes the inference types used in the previously described commonsense datasets. Although many of the existing inference types represent distinct commonsense information, we observed that there was significant overlap in several of the types that led to redundancy. In the rest of this section, we aim to identify the overlap between several synonymous inference types and explain the results of our synthesis of the general inference types.

\subsection{Effect} 

Inference type \texttt{Effect} comprises multiple types identified in the existing works: \texttt{Causes} from Atomic/ComFact, \texttt{xEffect} and \texttt{oEffect} from Atomic/Comfact, \texttt{Subsequent Events} from Cicero, and \texttt{Consequences} from Reflect. 

\paragraph{xEffect, oEffect, and Causes} \citet{hwang:21} acknowledge that inference types \texttt{xEffect} and \texttt{Causes} contain overlap in meaning, although they specify that \texttt{Causes} is also applicable to events that exist outside of human control (e.g. “bad weather” causes “power outages") whereas \texttt{xEffect} is specifically applicable to effects on humans, namely the person involved in the event. To this end, \texttt{Causes} can be viewed as a superset of \texttt{xEffect}, rendering it more generally applicable across a variety of situations in dialogue. Since \texttt{oEffect} is an analogous type to \texttt{xEffect} but applied to bystanders to the event, it also follows that \texttt{Causes} is a superset of \texttt{oEffect}. Thus, we choose to combine such instances into a single \texttt{Effect} inference type. 

\paragraph{Subsequent Events} \cite{ghosal:22} do not differentiate in causality when considering subsequent events of a premise; rather, their \texttt{Subsequent Event} inference type encapsulates both those events caused by the premise and those that are not directly caused by the premise. Thus, we include this inference type into \texttt{Effect} as well. 

\paragraph{Consequences} \citet{zhou:22} utilize a \texttt{Potential Consequences} inference type that captures events that are likely to follow the premise, which also is suitable for the \texttt{Effect} type.

% We hypothesized that there might be substantial overlap between \texttt{isBefore} and \texttt{Effect} as well. Although \texttt{Effect} targets the identification of subsequent events that are caused by the premise and \texttt{isBefore} does not, they both encapsulate the notion of events that are likely to follow the premise and it is unclear to what extent \texttt{isBefore} is distinct from \texttt{Effect} in practice.  To further assess their distinctness, we sampled 50 examples of both inference types from the ATOMIC10X dataset. ATOMIC10X is the only dataset that contains both inference types, thus controlling for differences in inference quality or format between different datasets that could confound the comparison. These examples were shown in random order to one of the authors, whose task was to categorize the example as an instance of \texttt{Effect} or the more general \texttt{isBefore}. We found a confusion rate of $\tilda30\%$ between the 2 labels.

% Choices:

% \begin{enumerate}
%     \item most of the \texttt{isBefore} examples were labelled as \texttt{Effect}, thus indicating that there is not a practical distinction between these two categories at least with their current definitions and implementations. We choose to merge \texttt{isBefore} into the \texttt{Effect} inference type for this work, as it is out of scope to investigate a higher acuity delineation of the differences between these types. 
%     \item the author matched the true categorizations of most the examples, thus indicating there is a meaningful and practical difference between these types that should be preserved.
% \end{enumerate}

\subsection{Cause} 

By their provided definitions, \texttt{xReason} used by \citet{hwang:21} is a synonym of the \texttt{Cause} inference type used by \citet{ghosal:22}. As a result, we treat them as one inference type: \texttt{Cause}.

\subsection{Prerequisite}

Inference types \texttt{xNeed} from Atomic/ComFact and \texttt{Prerequisites} from Cicero/Reflect exhibit a similar relationship to one another as \texttt{xEffect} and \texttt{Causes}, where \texttt{Prerequisites} can be viewed as a superset of \texttt{xNeed}. While \texttt{xNeed} is targets conditions related to the human that must be satisfied before the event can occur, \texttt{Prerequisites} is also applicable to events that exist outside of human control. We thus consider them to be one inference type: \texttt{Prerequisite}.

% \paragraph{Prerequisites and Cause}
% Furthermore, \citet{shen:22} acknowledge that the human annotators were unable to distinguish between \texttt{Prerequisites} and \texttt{Cause} inference types during the training process. 

\subsection{Excluded Types}

ComFact covers the all 23 inference types of \textbf{ATOMIC2020}; however, we focus on the inference types shown in Table \ref{tab:human-gen-datasets-types}. These types comprise all of the social- or event-related inferences, and exclude the physical-entity-focused inferences. We chose these types as they are the most relevant to common dialogue interactions and are most similar to the inference types covered by the dialogue-specific commonsense datasets described previously. 

Two of the event-related inferences in ComFact (and ATOMIC10X) are also excluded: \texttt{isBefore} and \texttt{isAfter}. These inference types capture a sense of the general temporal ordering of different events, without enforcing any notion of causation. For the purposes of dialogue, the causal aspect between events is more useful than a vague timeline and is already better captured through the \texttt{Cause} and \texttt{Effect} inference types. For this reason, we choose to exclude these lower acuity types in this work.







==> sections/old/generative_model_auto_eval.tex <==
\subsection{Automatic Evaluation}

There is likely a tradeoff between the reasonability and the diversity of the inferences outputted by generative commonsense models for dialogue, since the goal of generating multiple inferences for a single context can have a negative impact on the reasonability of the individual inferences that are generated. To quantify this impact grounded in practical usage scenarios, we perform evaluations under two representative paradigms:

\begin{itemize}
    \item 1-Best Generation: a single high-quality inference is desired.
    \item N-Best Generation: multiple high-quality and semantically diverse inferences are desired.
\end{itemize}

\subsubsection{Metrics}

As evaluation metrics, we use BLEU score, BertScore, and embedding similarity to assess how well the generations match the references.

\subsubsection{1-Best Generation}

We aim to measure the quality of the most probable inference generated by each model. The generation of a single high-probability inference follows directly from the design of the monomorphic models since they are trained to output a single inference at a time. Thus, to calculate the evaluation metrics for the monomorphic models, we directly compare the outputted inference to the references, and take the best match that results in the maximum score. On the other hand, since the polymorphic models output multiple inferences at a time, it is less straightforward the selection of the most probable inference. To this end, we report two strategies for evaluating a single inference for polymorphicc models:

\begin{itemize}
    \item Maximum Selection: we compare each inference from the generated list to each of the references, and take the maximum score.
    \item Order Selection: we compare the first generated inference (prefixed by \texttt{"(1)"} in the output) to each of the references, and take the maximum score.
\end{itemize}

\subsubsection{N-Best Generation}

It can be useful for many applications to generate a list of reasonable inferences that are applicable to the current dialogue context. In these situations, it is important for the inferences to be both reasonable to the context and semantically dissimilar to one another in order to present the most options possible. Even if the surface forms differ, inferences that are too semantically similar are not useful as individual inferences as they are repetitive in terms of their information. 

The ability to generate multiple inferences is a fundamental design principle of the polymorphic models, since they are trained to output a list of reasonable inferences for a given dialogue context and question. On the other hand, the monomorphic models are trained to output a single inference at a time. To obtain multiple inferences from a monomorphic model, we utilize the decoding strategy to output more than the most probably output. Specifically, we take the top-\textit{k} outputs from beam search decoding as the multiple generated inferences.

\paragraph{Diversity} To measure the diversity of the generated inferences, we perform clustering on the inferences generated by each model for a single dialogue and observe the sizes of the resultant groups. If each inference was semantically dissimilar, then each inference would belong to its own cluster, rather than being grouped with any of the other options. On the other extreme, if the inferences were all semantically identical, then this would result in a single cluster that contains all of the generated inferences. 

\paragraph{Reasonability} Through a manual analysis of both ConvoSense and the human-generated datasets, we find that the ground truth inferences for a single dialogue context are predominantly semantically distinct and can serve as appropriate references for this evaluation. Thus, we compare the generated inferences against the ground truth inferences present in the datasets in order to measure the reasonability of the generations. We calculate the maximum scores achievable by pairing the generations to the references in two settings:

\begin{itemize}
    \item Bipartite-Graph Matching: an injective mapping from generations to references (or references to generations, if the number of references is smaller than the number of generations). Each generation and reference can exist in only one match. This matching approach was proposed in (CITE) as a method to more appropriately measure generations that are supposed to be diverse from one another by disallowing more than one generation from matching to the same reference.
    \item Maximum Selection: although each generation is also paired to exactly one reference, this mapping is not injective. Instead, the same reference can be paired to more than one generation, if it results in the maximum score for those generations compared to the other reference options. 
\end{itemize}

We use the clustering results from the Diversity evaluation and only allow one generation from each cluster to be used during the evaluation metric calculations, where the generation is selected to optimize the evaluation metric score.

We perform the above evaluations for N-Best Generation under two variants of N: low and high. The \textbf{lowN} setting represents cases where a small number of inferences are desired such that the number generated in one run from the polymorphic model is adequate. The \textbf{highN} setting covers the situations where it is preferable to have a large number of inferences, which would practically require obtaining multiple runs of the polymorphic model in order to accumulate the desired quantity. To simulate these settings, we collect the inferences from one run of the polymorphic model for \textbf{lowN} setting and from three runs of the polymorphic model for \textbf{highN} setting for each example. For both of these settings, the monomorphic model output for each example is generated using beam search to match the size of the collected polymorphic outputs.

==> tab/data-eval-setup.tex <==

\begin{table}[ht]
    \centering
    \small 
    \SetTblrInner{rowsep=2pt,colsep=2pt}
    \begin{tblr}{
                    width=\textwidth,
                    hline{2-Y} = 0.5pt, vline{2-Y} = 0.5pt,
                    colspec = { X[1.8cm] | Q[c] Q[c] Q[c] Q[c] Q[c] | Q[c] Q[c] },
                    row{1} = {font=\bfseries},
                    column{1} = {font=\bfseries}
                }
                
Type & ATO & COM & CIC & REF & CS (A) & CS (MA) \\ \hline[0.5pt]

Effect & N & N & N & N & 4N & N\\

Cause & N & N & N & & 3N & N\\

Prerequisite & N & N & N & N & 4N & N\\

Motivation & N & N & N & & 3N & N\\

Attribute & N & N & & N & 3N & N\\

Reaction & N & N & & N & 3N & N\\

Reaction$_{o}$ & N & N & N & N & 4N & N\\

Desire & N & N & & & 2N & N\\

Desire$_{o}$ & N & N & & & 2N & N\\

Constituents &  & N & & & N & N\\

Obstacle & N & N & & & 2N & N\\

    \end{tblr}
    \caption{\textbf{ATO}: ATOMIC10X, \textbf{COM}: ComFact, \textbf{CIC(1/2)}: Cicero(v1/v2), \textbf{REF}: Reflect, \textbf{CS}: ConvoSense}
    \label{tab:data-eval-setup}
\end{table}

==> tab/data-human-generated-scale.tex <==

\begin{table}[ht]
    \centering
    \small 
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{c|c|c|c|c}
\toprule           
\bf Data & \bf Sources & \bf Dialogues & \bf Contexts & \bf Inferences \\ 
\midrule
% ATO & - & - & 165672 & 4739292\\
\bf COM & Mutual        & 339 & 1533 & 6246\\
    & PersonaChat   &       &       &   \\
    \midrule
\bf CIC & Mutual & 5673 & 25784 & 73689\\
    & DailyDialog   &       &       &   \\
    & DREAM   &       &       &   \\
    \midrule
% CIC2 & {subset CIC1} & 2379 & 4871 & 20485\\
\bf REF & Commonsense- & 599 & 599 & 3245\\
    & Dialogues   &       &       &   \\
    \bottomrule
    \end{tabular}
    }
    \caption{\small The number of unique dialogues (\textbf{Dialogues}), unique inference contexts (e.g. target utterance + dialogue context) (\textbf{Contexts}), and total inferences (\textbf{Inferences}) for the existing human datasets (\textbf{COM}: ComFact, \textbf{CIC}: Cicerov1+v2, \textbf{REF}: Reflect).} 
    % \vspace{}
    \label{tab:human-gen-datasets-scale}
\end{table}

==> tab/data-human-generated-types-old.tex <==

\begin{table*}[ht]
    \centering
    \small 
    \SetTblrInner{rowsep=2pt,colsep=2pt}
    \begin{tblr}{
                    width=\textwidth,
                    hline{2-Y} = 0.5pt, vline{2-Y} = 0.5pt,
                    colspec = { X[1.8cm] | X[1.9cm] | X Q[c] Q[c] Q[c] Q[c] },
                    row{1} = {font=\bfseries},
                    column{1} = {font=\bfseries}
                }
\toprule             
Type & Existing & Definition(s) & ATO & COM & CIC & REF \\ \hline[0.5pt]

Effect & {Causes \\ \\ xEffect \\ \\ oEffect \\ \\ Subsequent \\ Events \\ \\ Consequences} & {What does this event cause to happen? [2] \\ \\ What effect does the event have on X? [1] \\ \\ What effects does the event have on others? [1] \\ \\  What subsequent event happens or could happen following the Target? [3] \\ \\  What might happen after? [4] } & x & x & x & x \\

Cause & { xReason \\ \\ Cause} & {What could be the cause of this event? [2] \\ \\ What is the event that directly causes or could cause Target? [3]} & x & x & x & \\

Prerequisite & {xNeed \\ \\ Prerequisites} & {What does X need to do before the event can happen? [1] \\ \\ What is or could be the prerequisite of Target? [3] \\ What might have happened before? [4] } & x & x & x & x \\

Motivation & {xIntent \\ \\ Motivation} & {Why does X cause the event? [1] \\ \\ What is an emotion or basic human drive that motivates or could motivate Target? [3]} & x & x & x & \\

Attribute & xAttr & {How would X be described? [1] \\ How would you describe Speaker? [4] } & x & x & & x \\

Reaction & xReact & {How does X feel after the event? [1] \\ What is Speaker feeling now? [4]} & x & x & & x \\

Reaction$_{o}$ & oReact & {How do others feel after the event? [1] \\ What is the possible emotional reaction of the listener in response to target? [3] \\ What is Responder feeling now? [4]} & x & x & x & x \\

Desire & xWant & What would X likely want to do after the event? [1] & x & x & & \\

Desire$_{o}$ & oWant & What would others likely want to do after the event? [1] & x & x & & \\

Constituents & HasSubEvent & What is a substep that happens within this event? [2] &  & x & & \\

Obstacle & HinderedBy & What could obstruct the occurrence of this event? [2] & x & x & & \\
\bottomrule
    \end{tblr}
    \caption{The inference types covered in existing commonsense datasets (\textbf{ATO}: ATOMIC10X, \textbf{COM}: ComFact, \textbf{CIC}: Cicerov1/v2, \textbf{REF}: Reflect). Each row denotes a unique inference type. Rows which contain multiple type names in their \texttt{Existing} column represent semantic synthesis of multiple existing inference types into one (Sec. \ref{sec:type_synthesis}) using definitions and discussions from [1] \citet{sap:19}, [2] \citet{hwang:21}, [3] \citet{ghosal:22}, [4] \citet{zhou:22}. }
    \label{tab:human-gen-datasets-types}
\end{table*}

==> tab/old/auto_metrics.tex <==
\begin{table*}[htb!]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
 & \multicolumn{3}{c|}{\textbf{Top-1}} & \multicolumn{3}{c|}{\textbf{Top-5}} & \multicolumn{3}{c}{\textbf{Top-10}} \\
 & \bf BLEU & \bf BertScore & \bf Embed & \bf BLEU & \bf BertScore & \bf Embed & \bf BLEU & \bf BertScore & \bf Embed \\
\midrule
HumanGen-Mono & 8.9938 & 0.7097 & 0.5369 & 11.3403 & 0.7339 & 0.5955 & 13.0702 & 0.7491 & 0.6299\\
\midrule
HumanGen-Mono-DBS & 7.2021 & 0.6962 & 0.5098 & 9.8618 & 0.7337 & 0.6025 & 11.0549 & 0.7443 & 0.6294\\
\midrule
HumanGen-Poly & 7.0052 & 0.6721 & 0.4889 & 8.1637 & 0.6788 & 0.5179 & 8.1634 & 0.6914 & 0.526\\
\midrule
ConvoSense-Mono & 2.571 & 0.6405 & 0.4214 & 3.5175 & 0.6588 & 0.4746 & 4.3519 & 0.6696 & 0.5025 \\
\midrule
ConvoSense-Mono-DBS & 2.1797 & 0.6363 & 0.4154 & 3.8857 & 0.667 & 0.5091 & 4.9114 & 0.6792 & 0.5404 \\
\midrule
ConvoSense-Poly  & 2.3171 & 0.6339 & 0.4214 & 3.5422 & 0.6587 & 0.4981 & 3.5422 & 0.6588 & 0.4982\\  
\bottomrule
\end{tabular}
}
\caption{\small Results on HumanGen test split}
\label{tab:reference_eval_results}
\end{table*}

\begin{table*}[htb!]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
 & \multicolumn{3}{c|}{\textbf{Top-1}} & \multicolumn{3}{c|}{\textbf{Top-5}} & \multicolumn{3}{c}{\textbf{Top-10}} \\
 & \bf BLEU & \bf BertScore & \bf Embed & \bf BLEU & \bf BertScore & \bf Embed & \bf BLEU & \bf BertScore & \bf Embed \\
\midrule
HumanGen-Mono & 4.3679 & 0.6326 & 0.5005 & 1.4976 & 0.604 & 0.4247 & 1.8967 & 0.6246 & 0.4738\\
\midrule
HumanGen-Mono-DBS & 3.1892 & 0.6171 & 0.4813 & 1.0345 & 0.5862 & 0.4039 & 1.508 & 0.6137 & 0.4674\\
\midrule
HumanGen-Poly & 4.4196 & 0.5996 & 0.43 & 1.1317 & 0.5595 & 0.3945 & 1.1038 & 0.5849 & 0.413 \\
\midrule
ConvoSense-Mono & 23.6761 & 0.7774 & 0.7302 & 10.4145 & 0.7192 & 0.6192 & 12.3863 & 0.7389 & 0.665\\
\midrule
ConvoSense-Mono-DBS & 22.2466 & 0.7729 & 0.7253 & 11.7526 & 0.7287 & 0.6439 & 14.6619 & 0.7546 & 0.7056 \\
\midrule
ConvoSense-Poly  & 18.8012 & 0.7583 & 0.7025 & 10.4657 & 0.7212 & 0.6333 & 10.4657 & 0.7212 & 0.6333\\  
\bottomrule
\end{tabular}
}
\caption{\small Results on ConvoSense test split}
\label{tab:reference_eval_results}
\end{table*}

\^ Automatic metrics on full HumanGen data (without excluding the inferences not present in GPT data)







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table*}[htb!]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
 & \multicolumn{3}{c|}{\textbf{Top-1}} & \multicolumn{3}{c|}{\textbf{Top-5}} & \multicolumn{3}{c}{\textbf{Top-10}} \\
 & \bf BLEU & \bf BertScore & \bf Embed & \bf BLEU & \bf BertScore & \bf Embed & \bf BLEU & \bf BertScore & \bf Embed \\
\midrule
HumanGen-Mono & 9.0215 & 0.7106 & 0.5384 & 11.3662 & 0.7346 & 0.5965 & 13.0929 & 0.7496 & 0.6308\\
\midrule
HumanGen-Mono-DBS & 7.2263 & 0.6972 & 0.5112 & 9.8842 & 0.7344 & 0.6036 & 11.0783 & 0.7449 & 0.6304\\
\midrule
HumanGen-Poly & 7.6737 & 0.7003 & 0.5225 & 9.0076 & 0.7153 & 0.5632 & 9.0076 & 0.7153 & 0.5632\\
\midrule
ConvoSense-Mono & 2.5942 & 0.6413 & 0.4224 & 3.5427 & 0.6596 & 0.4755 & 4.3826 & 0.6704 & 0.5035 \\
\midrule
ConvoSense-Mono-DBS & 2.202 & 0.6371 & 0.4163 & 3.9135 & 0.6679 & 0.5101 & 4.9432 & 0.6801 & 0.5415 \\
\midrule
ConvoSense-Poly  & 2.3297 & 0.6347 & 0.4224 & 3.5619 & 0.6595 & 0.4993 & 3.5619 & 0.6596 & 0.4994\\  
\bottomrule
\end{tabular}
}
\caption{\small Results on HumanGen test split}
\label{tab:reference_eval_results}
\end{table*}

\begin{table*}[htb!]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
 & \multicolumn{3}{c|}{\textbf{Top-1}} & \multicolumn{3}{c|}{\textbf{Top-5}} & \multicolumn{3}{c}{\textbf{Top-10}} \\
 & \bf BLEU & \bf BertScore & \bf Embed & \bf BLEU & \bf BertScore & \bf Embed & \bf BLEU & \bf BertScore & \bf Embed \\
\midrule
HumanGen-Mono & 4.3679 & 0.6326 & 0.5005 & 1.4976 & 0.604 & 0.4247 & 1.8967 & 0.6246 & 0.4738\\
\midrule
HumanGen-Mono-DBS & 3.1892 & 0.6171 & 0.4813 & 1.0345 & 0.5862 & 0.4039 & 1.508 & 0.6137 & 0.4674\\
\midrule
HumanGen-Poly & 6.1742 & 0.6553 & 0.5282 & 3.993 & 0.647 & 0.5062 & 3.993 & 0.647 & 0.5062 \\
\midrule
ConvoSense-Mono & 23.6761 & 0.7774 & 0.7302 & 10.4145 & 0.7192 & 0.6192 & 12.3863 & 0.7389 & 0.665\\
\midrule
ConvoSense-Mono-DBS & 22.2466 & 0.7729 & 0.7253 & 11.7526 & 0.7287 & 0.6439 & 14.6619 & 0.7546 & 0.7056 \\
\midrule
ConvoSense-Poly  & 18.8012 & 0.7583 & 0.7025 & 10.4657 & 0.7212 & 0.6333 & 10.4657 & 0.7212 & 0.6333\\  
\bottomrule
\end{tabular}
}
\caption{\small Results on ConvoSense test split}
\label{tab:reference_eval_results}
\end{table*}



\^ incorrect bleu calculation


\begin{table*}[htb!]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
 & \multicolumn{3}{c|}{\textbf{Top-1}} & \multicolumn{3}{c|}{\textbf{Top-5}} & \multicolumn{3}{c}{\textbf{Top-10}} \\
 & \bf BLEU & \bf BertScore & \bf Embed & \bf BLEU & \bf BertScore & \bf Embed & \bf BLEU & \bf BertScore & \bf Embed \\
\midrule
ConvoSense-Mono & 5.4069 & 0.6413 & 0.4224 & 6.5165 & 0.6596 & 0.4755 & 7.2655 & 0.6704 & 0.5035 \\
\midrule
ConvoSense-Mono-DBS & 5.1306 & 0.6371 & 0.4163 & 6.9633 & 0.6679 & 0.5101 & 7.8572 & 0.6801 & 0.5415 \\
\midrule
ConvoSense-Poly & 4.9217 & 0.6347 & 0.4224 & 6.2523 & 0.6596 & 0.4994 & 6.2523 & 0.6596 & 0.4994 \\
\midrule
HumanGen-Mono & 10.7235 & 0.7106 & 0.5384 & 13.4275 & 0.7346 & 0.5965 & 15.1603 & 0.7496 & 0.6308 \\
\midrule
HumanGen-Mono-DBS & 9.473 & 0.6972 & 0.5112 & 12.5251 & 0.7344 & 0.6036 & 13.6589 & 0.7449 & 0.6304 \\
\midrule
HumanGen-Poly & 9.524 & 0.7003 & 0.5225 & 10.7905 & 0.7153 & 0.5632 & 10.7905 & 0.7153 & 0.5632 \\
\bottomrule
\end{tabular}
}
\caption{\small Results on HumanGen test split}
\label{tab:reference_eval_results}
\end{table*}

\begin{table*}[htb!]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
 & \multicolumn{3}{c|}{\textbf{Top-1}} & \multicolumn{3}{c|}{\textbf{Top-5}} & \multicolumn{3}{c}{\textbf{Top-10}} \\
 & \bf BLEU & \bf BertScore & \bf Embed & \bf BLEU & \bf BertScore & \bf Embed & \bf BLEU & \bf BertScore & \bf Embed \\
\midrule
ConvoSense-Mono & 19.0186 & 0.7774 & 0.7302 & 11.3964 & 0.7192 & 0.6192 & 13.5401 & 0.7389 & 0.665 \\
\midrule
ConvoSense-Mono-DBS & 17.9225 & 0.7729 & 0.7253 & 12.2413 & 0.7287 & 0.6439 & 15.0718 & 0.7546 & 0.7056 \\
\midrule
ConvoSense-Poly & 15.163 & 0.7583 & 0.7025 & 10.8931 & 0.7212 & 0.6333 & 10.8931 & 0.7212 & 0.6333 \\
\midrule
HumanGen-Mono & 5.0949 & 0.6326 & 0.5005 & 3.6599 & 0.604 & 0.4247 & 4.1399 & 0.6246 & 0.4738 \\
\midrule
HumanGen-Mono-DBS & 4.2625 & 0.6171 & 0.4813 & 3.1179 & 0.5862 & 0.4039 & 3.7764 & 0.6137 & 0.4674 \\
\midrule
HumanGen-Poly & 6.3584 & 0.6553 & 0.5282 & 5.8813 & 0.647 & 0.5062 & 5.8813 & 0.647 & 0.5062 \\
\bottomrule
\end{tabular}
}
\caption{\small Results on ConvoSense test split}
\label{tab:reference_eval_results}
\end{table*}


\^ without multianswer weighting for top-5 and top-10


\begin{table*}[htb!]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
 & \multicolumn{3}{c|}{\textbf{Top-1}} & \multicolumn{3}{c|}{\textbf{Top-5}} & \multicolumn{3}{c}{\textbf{Top-10}} \\
 & \bf BLEU & \bf BertScore & \bf Embed & \bf BLEU & \bf BertScore & \bf Embed & \bf BLEU & \bf BertScore & \bf Embed \\
\midrule
ConvoSense-Mono & 5.4069 & 0.6413 & 0.4224 & 6.2818 & 0.65 & 0.4623 & 7.0733 & 0.6651 & 0.4933 \\
\midrule
ConvoSense-Mono-DBS & 5.1306 & 0.6371 & 0.4163 & 6.7099 & 0.658 & 0.4962 & 7.6479 & 0.6747 & 0.5316 \\
\midrule
ConvoSense-Poly & 4.9217 & 0.6347 & 0.4224 & 6.0258 & 0.6451 & 0.4819 & 6.0258 & 0.6451 & 0.4819 \\
\midrule
HumanGen-Mono & 10.7235 & 0.7106 & 0.5384 & 12.7013 & 0.7215 & 0.5762 & 14.4568 & 0.741 & 0.6143 \\
\midrule
HumanGen-Mono-DBS & 9.473 & 0.6972 & 0.5112 & 12.0561 & 0.7238 & 0.5905 & 13.3151 & 0.7401 & 0.624 \\
\midrule
HumanGen-Poly & 9.524 & 0.7003 & 0.5225 & 9.6575 & 0.6448 & 0.5038 & 9.6575 & 0.6448 & 0.5038 \\
\bottomrule
\end{tabular}
}
\caption{\small Results on HumanGen test split}
\label{tab:reference_eval_results_humangen}
\end{table*}

\begin{table*}[htb!]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
 & \multicolumn{3}{c|}{\textbf{Top-1}} & \multicolumn{3}{c|}{\textbf{Top-5}} & \multicolumn{3}{c}{\textbf{Top-10}} \\
 & \bf BLEU & \bf BertScore & \bf Embed & \bf BLEU & \bf BertScore & \bf Embed & \bf BLEU & \bf BertScore & \bf Embed \\
\midrule
ConvoSense-Mono & 19.0186 & 0.7774 & 0.7302 & 11.1185 & 0.7001 & 0.6027 & 13.5854 & 0.739 & 0.6644 \\
\midrule
ConvoSense-Mono-DBS & 17.9225 & 0.7729 & 0.7253 & 11.9326 & 0.7093 & 0.6265 & 15.0927 & 0.7546 & 0.7046 \\
\midrule
ConvoSense-Poly & 15.163 & 0.7583 & 0.7025 & 9.7246 & 0.6437 & 0.5643 & 9.7246 & 0.6437 & 0.5643 \\
\midrule
HumanGen-Mono & 5.0949 & 0.6326 & 0.5005 & 3.5737 & 0.5881 & 0.4134 & 4.1624 & 0.6246 & 0.4728 \\
\midrule
HumanGen-Mono-DBS & 4.2625 & 0.6171 & 0.4813 & 3.0445 & 0.5708 & 0.3931 & 3.796 & 0.6136 & 0.4663 \\
\midrule
HumanGen-Poly & 6.3584 & 0.6553 & 0.5282 & 2.3297 & 0.2563 & 0.2005 & 2.3297 & 0.2563 & 0.2005 \\
\bottomrule
\end{tabular}
}
\caption{\small Results on ConvoSense test split}
\label{tab:reference_eval_results_convosense}
\end{table*}

\^ with top-10 column section




\begin{table}[htb!]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|ccc|ccc}
\toprule
 & \multicolumn{3}{c|}{\textbf{Top-1}} & \multicolumn{3}{c}{\textbf{Top-5}} \\
 & \bf BLEU & \bf BS & \bf Embed & \bf BLEU & \bf BS & \bf Embed \\
\midrule
ConvoSenseM & \bf 5.4069 & \bf 0.6413 & \bf 0.4224 & 6.2818 & 0.6500 & 0.4623 \\
ConvoSenseM* & 5.1306 & 0.6371 & 0.4163 & \bf 6.7099 & \bf 0.6580 & \bf 0.4962  \\
ConvoSenseP & 4.9217 & 0.6347 & \bf 0.4224 & 6.0258 & 0.6451 & 0.4819  \\
\midrule
HumanGenM & \bf 10.7235 & \bf 0.7106 & \bf 0.5384 & \bf 12.7013 & 0.7215 & 0.5762  \\
HumanGenM* & 9.473 & 0.6972 & 0.5112 & 12.0561 & \bf 0.7238 & \bf 0.5905  \\
HumanGenP & 9.524 & 0.7003 & 0.5225 & 9.6575 & 0.6448 & 0.5038  \\
\bottomrule
\end{tabular}
}
\caption{\small Reference metric results on HumanGen test. Columns \textbf{BS} denotes Bertscore.}
\label{tab:reference_eval_results_humangen}
\end{table}

\begin{table}[htb!]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|ccc|ccc}
\toprule
 & \multicolumn{3}{c|}{\textbf{Top-1}} & \multicolumn{3}{c}{\textbf{Top-5}} \\
 & \bf BLEU & \bf BS & \bf Embed & \bf BLEU & \bf BS & \bf Embed \\
\midrule
ConvoSenseM & \bf 19.0186 & \bf 0.7774 & \bf 0.7302 & 11.1185 & 0.7001 & 0.6027 \\
ConvoSenseM*& 17.9225 & 0.7729 & 0.7253 & \bf 11.9326 & \bf 0.7093 & \bf 0.6265 \\
ConvoSenseP & 15.163 & 0.7583 & 0.7025 & 9.7246 & 0.6437 & 0.5643 \\
\midrule
HumanGenM & 5.0949 & 0.6326 & 0.5005 & \bf 3.5737 & \bf 0.5881 & \bf 0.4134  \\
HumanGenM* & 4.2625 & 0.6171 & 0.4813 & 3.0445 & 0.5708 & 0.3931  \\
HumanGenP & \bf 6.3584 & \bf 0.6553 & \bf 0.5282 & 2.3297 & 0.2563 & 0.2005  \\
\bottomrule
\end{tabular}
}
\caption{\small Reference metric results on ConvoSense test. Columns \textbf{BS} denotes Bertscore.}
\label{tab:reference_eval_results_convosense}
\end{table}



\^ with 4 decimal points

==> tab/prompt-strategies.tex <==

\begin{table*}[t]
\centering
\small
\resizebox{\textwidth}{!}{
\begin{tabular}{c|p{20em}|c|p{20em}}
\toprule
\bf Strategy & \bf Context & \bf Type & \bf Inferences \\
\midrule
% {UF} & ...  & Cause & ...  \\
% &  (1) Speaker: The registration office . Did you bring your records with you ?  &  &  \ul{Listener: Yes .}  \\
% &  (2) Listener: Yes .  &  &  Speaker: Is anybody here with you ? Parents or siblings ?  \\
% &  (3) Speaker: Is anybody here with you ? Parents or siblings ?  &  &  (a) This was caused by being an independent adult.  \\
% &  (4) Listener: No , I'm here all by myself .  &  &  (b) This was caused by being away from family for work or school.  \\
% &  (5) Speaker: You are a brave kid . Go ahead to the registration office first , then to the doctors . &  &  (c) This was caused by a strained relationship with family members. \\
% \bf SS & (1) Speaker: You'll never believe what Cameron did today  & Cause & (a) This was caused by Cameron being unfamiliar with the game mechanics. \ul{(Cameron's lack of}  \\
%  &  (2) Listener: What did he do this time?  &  &  \ul{experience with the game caused him to quickly} \\
%  &  (3) Speaker: we were playing my favorite video &  & \ul{lose all the lives.)} \\
%  & game, and I let him use my avatar while I took a break  & & (b) This was caused by Cameron's overconfidence in his own abilities. \\
%  &  (4) Listener: let me guess, it did not end well  &  &  \ul{(Cameron likely underestimated the difficulty of}  \\
%  &  (5) \textit{Speaker: it took Cameron less than 10 minutes to lose all the lives I accumulated over two days of play} &  &  \ul{the game and overestimated his own skills.)} \\
% \midrule
\bf DL & (1) Listener: hi . how are you ? i just got back from a city council meeting .  & Motivation & (a) Speaker is motivated by their love for music and nostalgia.  \\
 &  (2) \textit{Speaker: hey i am good . whats that song the village people sang from the 70s ?}  &  &  (b) Speaker is motivated \ul{to stay fit and connected with their community by going to the gym.}  \\
 &  (3) Listener: ymca ? lol why do you ask ?  &  &  (c) Speaker is motivated \ul{to maintain their health} \\
 &  (4) Speaker: oh , its just the the gym that i work out at . how was the meeting ?  &  &  \ul{and support local businesses by eating organic, non-GMO food.} \\
 &  (5) Listener: so do you eat healthy too ? the only food i eat is locally sourced .  &  &  \\
 &  (6) Speaker: organic , non gmo , grass fed and finished . i like to eat during movies &  &  \\
\midrule
\bf AS & ...  & Desire & (a) Speaker has been wanting to take a swim class \\
 &  (1) Speaker: my mom had a cat name socks , mom died in 1979 , still miss her and the cat .  &  &  for a long time, and plans to sign up for one as soon as possible. \\
 &  (2) Listener: sorry to hear about your lost . i miss my family i am out of state studying dance  &  &  (b) \ul{Speaker recently heard about a fantastic swim class} and is excited to enroll in it soon.  \\
 &  (3) \textit{Speaker: lucky you ! if i could i would take a swim class to learn how .} &  & (c) \ul{Speaker's friend recommended a great swim class}, and they are considering giving it a try. \\
\bottomrule
\end{tabular}
}
\caption{\small Prototypical examples of the erroneous behaviors observed for different GPT prompt strategies (\textbf{UF}: Utterance Focus, \textbf{SS}: Span Selection, \textbf{DL}: Dialogue Lookahead, \textbf{AS}: Answer Scope). The target utterance of the inference generation for each example is shown in \textit{italics}. The erroneous inferences are \underline{underlined}.}
\label{tab:gpt-prompt-strategies}
\end{table*}
